Differentially Private Grids for Geospatial Data

In this paper, we tackle the problem of constructing a differentially private synopsis for two-dimensional datasets such as geospatial datasets. The current state-of-the-art methods work by performing recursive binary partitioning of the data domains, and constructing a hierarchy of partitions. We show that the key challenge in partition-based synopsis methods lies in choosing the right partition granularity to balance the noise error and the non-uniformity error. We study the uniform-grid approach, which applies an equi-width grid of a certain size over the data domain and then issues independent count queries on the grid cells. This method has received no attention in the literature, probably due to the fact that no good method for choosing a grid size was known. Based on an analysis of the two kinds of errors, we propose a method for choosing the grid size. Experimental results validate our method, and show that this approach performs as well as, and often times better than, the state-of-the-art methods. We further introduce a novel adaptive-grid method. The adaptive grid method lays a coarse-grained grid over the dataset, and then further partitions each cell according to its noisy count. Both levels of partitions are then used in answering queries over the dataset. This method exploits the need to have finer granularity partitioning over dense regions and, at the same time, coarse partitioning over sparse regions. Through extensive experiments on real-world datasets, we show that this approach consistently and significantly outperforms the uniform-grid method and other state-of-the-art methods.

==> 2dpub.tex <==
%!TEX root = ./md_hist.tex


If we have data where each dimension is continuous in the range [0,1], there are two sources of error that influence the utility of the resultant synthetic anonymized data. These errors arise due to partitioning the data into discrete bins and releasing the count of each bin. Intuitively, we would like to partition the attribute domain into bins with the smallest area while satisfying differential privacy and ensuring that the distribution of data points in each bin is as uniform as possible.

$$E_t = E_{DP} + E_{u}$$

$$\textrm{error} = \int_0^1 d(x) - T\cdot x$$

Algorithm is simple: coarsely partition the data into $N$ regions and obtain a noisy count for each region. If the count exceeds a particular threshold, recursively partition that region. Otherwise, recalculate count using remaining $\epsilon$. Finally, perform constrained inference.

We tackle the problem of publishing two dimensional data...

The range query resulting in the largest error is the one that is slightly smaller than the total region. All non-boundary partitions are fully included boundary partitions are partially included.

Analysis for 1 grid: Assume that the grid is divided into $m \times m$ regions. Hence, there are $4m-4$ boundary regions. The errors are as follows:

\begin{itemize}
	\item Error due to differential privacy. We will be querying $m^2$ partitions at most. The standard deviation of the error for each differentially private query is $\frac{\sqrt{2}}{\epsilon}$, and this error is additive. Thus,
		$$E_{DP} \leq m^2 \cdot \frac{\sqrt{2}}{\epsilon}$$
	\item Error due to non-uniformity. Assume we have a fixed non-uniformity factor $f$, where $f=0$ means that the data points are uniformly distributed in the region, and $f=1$ indicates a maximally skewed distribution. 
		$$E_{u} \leq f \cdot (4m-4) \cdot \frac{N}{m^2}$$
\end{itemize}

\begin{align*}
	E &\leq m^2 \cdot \frac{\sqrt{2}}{\epsilon} + f \cdot (4m-4) \cdot \frac{N}{m^2} \\ 
	  &\leq m^2 \cdot \frac{\sqrt{2}}{\epsilon} + \frac{4fN}{m}
\end{align*}

\begin{align*}
	\frac{d}{d m}E &= 2m \cdot \frac{\sqrt{2}}{\epsilon} - \frac{4fN}{m^2} = 0 \\
							m^3 &= \sqrt{2}fN\epsilon\\
							m &= \sqrt[6]{2}\sqrt[3]{fN\epsilon} 							
\end{align*}



\subsection{Single Dimension}

Single Dimension: Divide the range into $m$ partitions

\begin{itemize}
	\item Error due to differential privacy. We will be querying $m$ partitions at most. The variance of the error for each differentially private query is $\frac{2}{\epsilon^2}$, and this error is additive. Thus,
		$$E_{DP} \leq m \cdot \frac{2}{\epsilon^2}$$
	\item Error due to non-uniformity. Assume we have a fixed non-uniformity factor $f$, where $f=0$ means that the data points are uniformly distributed in the region, and $f=1$ indicates a maximally skewed distribution. Non-uniformity will affect the result of at most 2 regions included in the query. Each region is expected to have $\frac{N}{m}$ points. Hence, the expected error square is
		$$E_{u} \leq 2\left(f \cdot \frac{N}{m}\right)^2$$
\end{itemize}

\begin{align*}
	E &\leq m \cdot \frac{2}{\epsilon^2} + 2\left(f \cdot \frac{N}{m}\right)^2
\end{align*}

\begin{align*}
	\frac{d}{d m}E &= \frac{2}{\epsilon^2} - \frac{4f^2N^2}{m^3} = 0 \\
							m^3 &= 2f^2N^2\epsilon^2\\
							m &= (2f^2N^2\epsilon^2)^\frac{1}{3}
\end{align*}

Hence, %\todo{modify}

\begin{align*}
		E &\leq (2f^2N^2\epsilon^2)^\frac{1}{3}  \cdot \frac{2}{\epsilon^2} + 2f \cdot \frac{N}{(2f^2N^2\epsilon^2)^\frac{1}{3}}\\
		  &\leq
\end{align*}

%\begin{align*}
%		E &\leq 2^{1/4}\sqrt{fN\epsilon}  \cdot \frac{\sqrt{2}}{\epsilon} + 2f \cdot \frac{N}{2^{1/4}\sqrt{fN\epsilon} }\\
%		  &\leq 2^{7/4}\frac{\sqrt{fN}}{\sqrt{\epsilon}}
%\end{align*}


\paragraph{Can we allow 2 cuts?}

For simplicity, assume all second levels cuts divide the area into $m_2$ regions

\begin{itemize}
	\item Error due to differential privacy
		$$E_{DP} \leq (m_1-2) \cdot \frac{2}{\epsilon_1^2} +  2(m_2-1) \cdot \frac{2}{\epsilon_2^2}$$
	
	\item Error due to non-uniformity
		$$E_u \leq 2\left(f_1 f_2 \cdot \frac{N}{m_1 m_2}\right)^2$$
\end{itemize}

\begin{align*}
	E &\leq (m_1-2) \cdot \frac{2}{\epsilon_1^2} +  2(m_2-1) \cdot \frac{2}{\epsilon_2^2} + 2\left(f_1 f_2 \cdot \frac{N}{m_1 m_2}\right)^2
\end{align*}

\paragraph{relative error}.

Can we optimize for the relative error? Optimizing seems to yield the same result.

\begin{itemize}
	\item DP error is
		$$E_{DP} \leq \frac{m}{N} \cdot \frac{\sqrt{2}}{\epsilon}$$
		
	\item non-uniformity error is
		$$E_{u} \leq 2f \cdot \frac{1}{m}$$
\end{itemize}

\begin{align*}
	E &\leq \frac{m}{N} \cdot \frac{\sqrt{2}}{\epsilon} + 2f \cdot \frac{1}{m}
\end{align*}

\begin{align*}
	\frac{d}{d m}E &= \frac{\sqrt{2}}{N\epsilon} - \frac{2f}{m^2} = 0 \\
							m^2 &= \sqrt{2}fN\epsilon\\
							m &= 2^{1/4}\sqrt{fN\epsilon} 							
\end{align*}


\paragraph{Recursive partitioning}


==> analysis.tex <==
\section{Open Problems}


In general, in low-dimensional publishing, given a cell that has negative count, we want to turn it to 0, and then propagates it to the nearby nodes, with the following properties.

\section{Analysis}

Suppose that we have a set of $n$ unit bins.  We are interested in optimizing for a set $Q$ of queries, and we assume some probability distribution $\mathbf{p}$ of the queries.

The queries can be represented using a $m\times n$ matrix $Q$, where each entry is $1$ or $0$.

There are several dimensions of the problem to consider:

\begin{itemize}
 \item
Absolute error or relative error.

 \item
Worst-case of average case.

 \item
Bounding error variance or error.  Requiring bounding for all error makes no sense.
\end{itemize}

Suppose that we care about average case.

In flat case, the average error is $(Q \mathbf{1})^T \mathbf{p}$.  Under what circumstance can one do better?

A mechanism is

When combining two bins into one and issue a new query for them, queries involving only that bin suffer by a factor of $\frac{1}{\epsilon_1^2}$, and queries involving both bins benefit, we need to count their probabilities.
For $m=2^{n}$ and $\mathbf{p}$  uniform.  There are $2^{n-1}$ queries that include only one bin, but not the other, and $2^{n-2}$ queries that include both.

For one-dimensional, there are a total of $n(n+1)/2$ queries, the number of queries including $b$ consecutive bins $j,j+1,j+b-1$ is $j*(n+1-b)$, the average of this is $(n+1)(n+1-b)/2$, and the number of queries including only part of the $b$ bins is $(b-1)*n$.

For two-dimensional, we assume a square domain, there are a total of $((\sqrt{n}+1)(\sqrt{n})/2)^2\approx n^2/4$ queries.  For any $b$ consecutive bins, the number of queries

Very quickly, the best method is going to be flat.

\mypara{What is the optimal Flat Method Grid size?}

\mypara{What is the optimal }

\mypara{Consider a special case of publishing noisy bin counts while minimizing normalized SSE.}  Given a sparse dataset, compare the following methods: (1) flat, (2) turn negative to $0$, (3), small region enforcing non-negativity (while maintaining small region sum), (4) one global

\mypara{Perspective.}  Differentially private data publishing is an problem in optimal adaptive experimental design in parameter estimation.

\begin{itemize}
 \item
Given a set of queries, one's goal is to estimate the underlying data when the answers are noisy.  This is a parameter estimation problem.

When Laplace noise is used, the MLE estimation does not seem to give a unique solution.

When we consider non-negativity constraint, we want to do MAP inference.

 \item


\end{itemize}

\section{Adaptive Design}

While one can view the problem as a design problem, the problem is really an adaptive design.

\subsection{Bottom-up Approach}

For one-dimensional data, the approach works as follows:

\begin{itemize}
 \item
For each unit range, issue a query.  If the density is too high, further divide.  If the density is medium, issue another query.  Otherwise, merge into a larger range, and issue another query.
\end{itemize}

\section{Least Norm?}

We may try to view the problem as a Least Norm problem.  However, we have a non-negativity constraint.

One way to view the problem of publishing synthetic dataset while satisfying all the marginal tables is to view this as a Least Norm problem.  We can view all the cells in the full contingency table as a vector x, and we know the complete sum and a number of partial sums about these cells.  These can be written as Ax=y, where each row of A specifies which cells are to be summed together for one sum.  These partial and complete sums, however, do not fully determine the cells, and there are many solutions.  I think it makes sense to want the least-form solution.

While there are numerical solution to the least-norm problem, I am not sure whether the fact that all values are

I've also been thinking we should try the following multiplicative update method (additive updates do not respect the non-negativity constraint).

First step, we compute all the intersecting marginal tables between the known ones and the target one (the one to be generated); these form all constraints that we respect.  If we want to generate the full contingency table, then the constraint marginal tables are exactly the known ones.

Start from the uniform distribution, each constraint marginal table divides the cells into budgets, get the count from the target table and the constraint table, and then multiple each cell in the target table by the corresponding scale factor to make it the same as the constraint table.

Repeat this until it converges.

\section{Old Text}

Many data publishing mechanisms that are differently private follow the Partitioning and Summarization (P\&S) approach.  That is, the dataset is partitioned into mutually disjoint regions, then one publishes the regions and the number of data points in each region in a differentially private way.

This approach is natural for the following reasons.  First, count queries have low sensitivity and can be answered relatively accurately.  Second, adding or removing a single data point affects the counts of at most one of the disjoint regions, hence each query can use the total privacy budget.

\paragraph{Two Utility Measurement}

We consider accuracy of (possibly multi-dimensional) range queries as the utility measurement for data publishing. One could consider either absolute error or relative error.

We are measuring the average error for queries of particular length.

We want to minimize $E[Var(Err_{\ell})]$

\todo{Needs a series of definition to define the error measurements.}

$Err_{\ell})$ is given the method, dataset, a random query of length $\ell$ is chosen, assuming that all equal length queries are equally likely.

\paragraph{Two Sources of Errors}

We call them \emph{noise error} and \emph{non-uniformity error}.

In general, noise error is determined on how many cells are

\paragraph{Three parameters.}

\subsection{Optimizing for Absolute Errors}

Top-level decision.  Branching factor $b$. 

==> background.tex <==
%!TEX root = ./md_hist.tex

\begin{comment}
\subsection{Differential Privacy}

The notion of differential privacy, which was developed in a series of papers~\cite{DN03,DN04,BDMN05,DMN+06,Dwo06}, represents a major breakthrough in private data analysis. The intuition behind this privacy notion is as follows: if a disclosure occurs when an individual participates in the database, then the same disclosure also occurs with similar probability (within a small multiplicative factor) even when the individual does not participate. %More formally, differential privacy requires that, given two input datasets that differ only in one tuple, the output distributions of the algorithm on these two datasets should be close.

\begin{definition}[$\epsilon$-Differential Privacy, \eDP ~\cite{Dwo06,DMN+06}] \label{def:diff}
A randomized algorithm $\AA$ gives $\epsilon$-differential privacy if for any pair of neighboring datasets $D$ and $D'$, and any $S\in \mathit{Range}(\AA)$,
%\lbskip
\begin{equation}\label{eqn:dp}
%e^{-\epsilon}   \leq \frac{\Pr[\AA(D)=S]}{\Pr[\AA(D')=S]} \leq e^{\epsilon}
\Pr{\AA(D)=S} \leq e^{\epsilon}\Pr{\AA(D')=S}
\end{equation}
\end{definition}

The parameter $\epsilon$ measures the degree of privacy.  The larger $\epsilon$ is, the lower the privacy.  When $\epsilon$ is too large, the privacy guarantee becomes meaningless.  Hence one needs to have a limit for $\epsilon$, which is know as a \emph{privacy budget}.  Answering each query consumes a portion of privacy budget.   When the privacy budget is used up after answering a number of queries, no new queries can be answered.

To satisfy differential privacy, one adds noise proportional to the maximum change any individual can make to the output of the query function, $f$. This is generally referred to as the \emph{global sensitivity} ($\mathsf{GS}_f$) or the $L_1$ sensitivity of the function $f$, defined as %follows:
%
%\begin{definition}[Global Sensitivity~\cite{Dwo06}]
% 	For a function $f: \mathcal{D} \rightarrow \mathcal{R}^d$, the global sensitivity of $f$ is
		$ \mathsf{GS}_f(D) = \max_{D, D'} ||f(D) - f(D')||_1 $
	for all $D$, $D'$ differing in at most one element.
%\end{definition}

%Note that this is in contrast to the \emph{local sensitivity} ($\mathsf{LS}_f(D)$) of a function which only considers the maximum change relative to a fixed dataset $D$.

%It is known that by adding carefully chosen noise with a standard deviation proportional to the global sensitivity to the output of the function, we can satisfy differential privacy.
\begin{theorem}[Laplace Mechanism~\cite{Dwo06,DMN+06}]
	A privacy mechanism $\AA_f$, for query function $f$,
	$$\AA_f(D)=f(D)+\mathsf{Lap}\left(\frac{\mathsf{GS}_f}{\epsilon}\right),$$
	that computes $f(D)$ and then adds noise sampled from the Laplace distribution with standard deviation $\mathsf{GS}_f/\epsilon$ satisfies $\epsilon$-differential privacy.
\end{theorem}
\end{comment}


Differential privacy has been widely accepted in the research community as the notion of choice for private data analysis.

\begin{definition}[{$\epsilon$-Differential Privacy~\cite{Dwo06,DMNS06}}] \label{def:diff}
A randomized mechanism $\AA$ gives $\epsilon$-differential privacy if for any pair of neighboring datasets $D$ and $D'$, and any $S\in \mathit{Range}(\AA)$,
%\begin{equation}\label{eqn:dp}
$$\Pr{\AA(D)=S} \leq e^{\epsilon}\cdot \Pr{\AA(D')=S}.$$
%\end{equation}
\end{definition}

In this paper we consider two datasets $D$ and $D'$ to be neighbors if one dataset equals the other dataset with one additional tuple added. We use $D\simeq D'$ to denote this.

Differential privacy is composable in the sense that combining multiple mechanisms that satisfy differential privacy for $\epsilon_1, \cdots,\epsilon_m$ results in a mechanism that satisfies $\epsilon$-differential privacy for $\epsilon=\sum_{i} \epsilon_i$.  Because of this, we refer to $\epsilon$ as the privacy budget of a privacy-preserving data analysis task.  When a task involves multiple steps, the budget is divided for different steps to use.

%Jason:
%The first method is to add random noise proportional to $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_1$ sensitivity of the function $g$.
One mechanism for satisfying $\epsilon$-differential privacy is to add to the output of a function $g$ random noise proportional to $\mathsf{GS}_f$, where $\mathsf{GS}_f$ is the \emph{global sensitivity} or the $L_1$ sensitivity of $g$. Such a mechanism to randomize the output of function $g$ (defined on a database $D$) can be denoted by $\AA_g$:
$$
\begin{array}{crl}
& \AA_g(D) & =g(D)+\mathsf{Lap}\left(\frac{\mathsf{GS}_g}{\epsilon}\right)
  \\
\mbox{where} &  \mathsf{GS}_g & = \max_{D\simeq D'} |g(D) - g(D')|,
\\
\mbox{and}& \Pr{\Lapp{\beta}=x} & = \frac{1}{2\beta} \myexp{-|x|/\beta}
\end{array}
$$
In the above, $\Lapp{\beta}$ represents a random variable sampled from the Laplace distribution with scale parameter $\beta$. This is generally referred to as the \emph{Laplacian mechanism} for satisfying differential privacy.


\begin{comment}
\subsection{Multidimensional Data Publishing}

In this paper, we consider the case of publishing a multidimensional dataset with differential privacy.

We denote a dataset consisting of $n$ dimensions by $\DD^n$. Throughout the paper, we focus our analysis on datasets with binary attributes. It should be noted, however, that our approach can be easily extended beyond this restriction.

We assume the existence of a class queries, $Q$, a subset of which that the data analyst is interested in obtaining accurate answers to. Each query, $q \in Q$, specifies conditions on a subset of the attributes. We refer to the number of attributes that the query considers as the \emph{width} of the query, and use $Q_w$ to denote the class of all queries of width $w$. When applied on the dataset $\DD$, $q$ returns the number of records that satisfy the query conditions.% $q: x \in D \rightarrow \{0,1\}$ maps a record from the dataset to the set to the domain $\{0,1\}$
%Since the data publisher may not know what queries are going to be asked,

\begin{table*}
	\centering
	\subfigure[]{
	\begin{tabular}{c|c|c|c}
		 record \# & a & b & c \\ \hline
		1 & 1 & 1 & 0 \\ \hline
		2 & 1 & 1 & 1 \\ \hline
		3 & 0 & 0 & 1 \\ \hline
		4 & 0 & 1 & 1 \\ \hline
		5 & 0 & 1 & 1 \\ \hline
		6 & 1 & 0 & 0 \\ \hline
		7 & 1 & 1 & 0 \\ \hline
		8 & 1 & 0 & 0 \\ \hline
		9 & 1 & 0 & 1 \\ \hline
	\end{tabular}
	}%\hfill
	\subfigure[]{
	\begin{tabular}{c|c|c||c}
	 	a & b & c & count \\ \hline
		0 & 0 & 0 & 0 \\ \hline
	 	0 & 0 & 1 & 0 \\ \hline
	 	0 & 1 & 0 & 0 \\ \hline
		0 & 1 & 1 & 0 \\ \hline
		1 & 0 & 0 & 0 \\ \hline
		1 & 0 & 1 & 0 \\ \hline
		1 & 1 & 0 & 0 \\ \hline
		1 & 1 & 1 & 0 \\ \hline
	\end{tabular}
	}
	\label{}
	\caption{Dataset with 3 binary attributes. Contingency table. Cells that need to be added to answer query $q = ?$ are highlighted}
\end{table*}


The basic, and most ubiquitous, approach to publishing a multidimensional dataset, henceforth referred to as the Flat method ($\F$), adds noise to all counts in the contingency table of the dataset. Since removing any record can affect at most one count in the contingency table, we can satisfy \eDP by adding noise from $\Lap\left(\frac{1}{\epsilon}\right)$.

THe variance of the Laplace distribution with scale $\lambda$ is $2\lambda^2$. Hence, the noise added to each cell has a variance of $\frac{2}{\epsilon^2}$. To answer any query, $q \in Q_w$, one has sum the noisy counts in the cells relevant to the query.

%$$\MaxV[\F, w] = 2^{} $$
\end{comment}





==> related.tex <==
%!TEX root = ./md_hist.tex




